Trajectory Planning with Model Predictive Control for Obstacle Avoidance Considering Prediction Uncertainty

This paper introduces a novel trajectory planner for autonomous robots, specifically designed to enhance navigation by incorporating dynamic obstacle avoidance within the Robot Operating System 2 (ROS2) and Navigation 2 (Nav2) framework. The proposed method utilizes Model Predictive Control (MPC) with a focus on handling the uncertainties associated with the movement prediction of dynamic obstacles. Unlike existing Nav2 trajectory planners which primarily deal with static obstacles or react to the current position of dynamic obstacles, this planner predicts future obstacle positions using a stochastic Vector Auto-Regressive Model (VAR). The obstacles' future positions are represented by probability distributions, and collision avoidance is achieved through constraints based on the Mahalanobis distance, ensuring the robot avoids regions where obstacles are likely to be. This approach considers the robot's kinodynamic constraints, enabling it to track a reference path while adapting to real-time changes in the environment. The paper details the implementation, including obstacle prediction, tracking, and the construction of feasible sets for MPC. Simulation results in a Gazebo environment demonstrate the effectiveness of this method in scenarios where robots must navigate around each other, showing improved collision avoidance capabilities.

==> Figures/control_structure.tex <==
\begin{tikzpicture}[node distance = 0.5cm, auto]
\node[block] (path_planner) {Path Planner};
\node[block, below=of path_planner] (trajectory_planner) {Trajectory Planner};
\node[block, below=of trajectory_planner] (controller) {Low-Level Controller};
\node[block, below=of controller] (robot) {Robot};
\node[knoten, below=of robot] (out) {};
\node[below=of out] (final) {};
\node[block, left= of robot] (observer) {Observer};
\node[knoten, above=0.85cm and 0.0cm of observer] (knoten) {};
\path[pfeil] (path_planner) -> (trajectory_planner) node [right, midway] {path};
\path[pfeil] (trajectory_planner) -> (controller) node [right, midway] {trajectory};
\path[pfeil] (controller) -> (robot) node [right, midway] {input};
\path[pfeil] (robot) -> (out);% node [right, midway] {sensor data};
\path[pfeil] (out) -> (final) node [right, midway] {sensor data};
\path[pfeil] (out) -| (observer) node [left, midway] {};
\path[pfeil] (observer) -- (knoten) node [left, midway] {estimated state};
\path[pfeil] (knoten) |- (trajectory_planner) node [left, midway] {};
\path[pfeil] (knoten) -- (controller) node [left, midway] {};
\end{tikzpicture}

==> Figures/details_control_structure.tex <==
\begin{tikzpicture}[node distance = 0.5cm, auto]
\node[block] (path_planner) {Path Planner};
\node[block, below=1.6cm and 0cm of path_planner] (trajectory_planner) {Trajectory Planner};
\node[block, below=1.6cm and 0cm of trajectory_planner] (controller) {Controller};
\node[block, above right=0.5cm and -0.5cm of path_planner] (VAR) {Obstacle Prediction};
\node[block, below=1.6cm and 0cm of VAR] (set_construction) {Set Construction};
\node[block, below=of controller] (robot) {Robot};
\node[knoten, below=of robot] (out) {};
\node[below=of out] (final) {};
\node[block, above left=0.35cm and -0.5cm of controller] (observer) {Extended Kalman Filter};
\node[knoten, above=0.65cm and 0cm of observer] (left_of_trajectory) {};
\node[sum, above=of controller] (summe) {};
\node[right=1.95cm and 1.95cm of summe] (meetme) {};
\node[below right=of summe, xshift=-0.5cm, yshift=0.5cm] (minus) {$-$};
\node[block, left=0.0cm and 1.7cm of VAR] (obstacle_tracker) {Obstacle Tracking};
\path[pfeil] (path_planner) -> (trajectory_planner) node [left, midway] {$\begin{pmatrix} \matvar{p}_{r,k+1} \\ \vdots \\ \matvar{p}_{r,k+N} \end{pmatrix}$};
\path[pfeil] (trajectory_planner) -> (summe) node [right, midway] {$\matvar{X}_{r,k}$};
\path[pfeil] (VAR) -> (set_construction) node [right, midway] {$\begin{Bmatrix} \left\{\matvar{\mu}_{k+1}, \matvar{\Sigma}_{k+1}\right\}, \\ \vdots \\ \left\{\matvar{\mu}_{k+N}, \matvar{\Sigma}_{k+N}\right\} \end{Bmatrix}_d$};
\draw[-latex'] (set_construction.south) |- (trajectory_planner.east) node [right, midway] {$\bigcap_d \mathbb{D}_{d,k+i}^\complement$};
\draw[pfeil] (observer.north) -> (left_of_trajectory) node [left, midway] {$\hat{\matvar{x}}_{k}$};
\draw[pfeil] (left_of_trajectory) -> (trajectory_planner);
\draw[-latex'] (left_of_trajectory) |- (path_planner);
\draw[pfeil] (robot) -> (out) node [right, midway] {$\matvar{y}_{k}$};
\draw[-latex'] (out) -| (observer);
\draw[pfeil] (out) -> (final);
\draw[pfeil] (controller) -> (robot);
\draw[pfeil] (summe) -> (controller);
\draw [] (out) -| ($ (meetme) + (0,0.005) $);
\draw [pfeil] ($ (meetme) + (0.005,0.0) $) -- (summe);
\draw [pfeil] (obstacle_tracker) -- (VAR) node [above, midway] {obstacle} node[below, midway]{positions};
\end{tikzpicture}

==> Figures/ellipse_and_circles.tex <==
\begin{tikzpicture}
    % variables
    \def\rotationvalue{25}
    \def\expectedx{2}
    \def\expectedy{2}
    \def\scalingminor{0.8}
    \def\scalingmajor{2.5}
    \def\distance{1.3}
    % Draw the coordinate system
    \draw[pfeil] (-1,0) -- (3,0) node[below] {$\prescript{}{0}{x}$};
    \draw[pfeil] (0,-1) -- (0,3) node[left] {$\prescript{}{0}{y}$};
    % Draw the ellipse centered at (1,1)
    \draw[black] (\expectedx,\expectedy) ellipse [x radius=\scalingmajor cm, y radius=\scalingminor cm, rotate=\rotationvalue];
    \fill[chemorange, opacity=0.1] (\expectedx,\expectedy) ellipse [x radius=\scalingmajor cm, y radius=\scalingminor cm, rotate=\rotationvalue];
    \draw[black] (\expectedx,\expectedy) ellipse [x radius={\scalingmajor+\distance}, y radius={\scalingminor+\distance}, rotate=\rotationvalue];
    \fill[wiwirot, opacity=0.1] (\expectedx,\expectedy) ellipse [x radius={\scalingmajor+\distance}, y radius={\scalingminor+\distance}, rotate=\rotationvalue];
    % Optional: grid for reference
    % Draw eigen-vectors
    % major
    \draw[loosely dotted, wiwirot] ({\expectedx - cos(\rotationvalue)*(\scalingmajor+\distance)}, {\expectedy - sin(\rotationvalue)*(\scalingmajor+\distance)}) -- ({\expectedx + cos(\rotationvalue)*(\scalingmajor+\distance)}, {\expectedy + sin(\rotationvalue)*(\scalingmajor+\distance)});
    \draw[loosely dotted, wiwirot] ({\expectedx - cos(\rotationvalue+90)*(\distance+\scalingminor)}, {\expectedx - sin(\rotationvalue+90)*(\distance+\scalingminor)}) -- ({\expectedx + cos(\rotationvalue+90)*(\distance+\scalingminor)}, {\expectedx + sin(\rotationvalue+90)*(\distance+\scalingminor)}); 
    \fill[wiwirot] (\expectedx,\expectedy) circle (2pt); 
    \def\radiusObstacle{0.5};
    % middle robot/obstacle
    \def\radiusRobot{\distance-\radiusObstacle};
    \draw[black] ({\expectedx + cos(\rotationvalue+90)*\scalingminor},{\expectedy+sin(\rotationvalue+90)*\scalingminor}) circle (\radiusObstacle) node[above] {obstacle};
    \filldraw    ({\expectedx + cos(\rotationvalue+90)*\scalingminor},{\expectedy+sin(\rotationvalue+90)*\scalingminor}) circle (1pt);
    \draw[black] ({\expectedx + cos(\rotationvalue+90)*(\scalingminor+\distance)},{\expectedy+sin(\rotationvalue+90)*(\scalingminor+\distance)}) circle (\radiusRobot) node [above]{robot};
    % Left robot/obstacle
    \filldraw    ({\expectedx + cos(\rotationvalue+90)*(\scalingminor+\distance)},{\expectedy+sin(\rotationvalue+90)*(\scalingminor+\distance)}) circle (1pt);
    \draw[black] ({\expectedx + cos(\rotationvalue+180)*\scalingmajor},{\expectedy+sin(\rotationvalue+180)*\scalingmajor}) circle (\radiusObstacle) node [above] {obstacle};
    \filldraw    ({\expectedx + cos(\rotationvalue+180)*\scalingmajor},{\expectedy+sin(\rotationvalue+180)*\scalingmajor}) circle (1pt);
    \draw[black] ({\expectedx + cos(\rotationvalue+180)*(\scalingmajor+\distance)},{\expectedy+sin(\rotationvalue+180)*(\scalingmajor+\distance)}) circle (\radiusRobot) node [above]{robot};
    %
    \filldraw    ({\expectedx + cos(\rotationvalue+180)*(\scalingmajor+\distance)},{\expectedy+sin(\rotationvalue+180)*(\scalingmajor+\distance)}) circle (1pt);
    %
    % circles (off axis), that show imperfection
    % rotation matrix:
    \def\ROneOne{+cos(\rotationvalue)}; % entry R_11 of rotation matrix
    \def\ROneTwo{-sin(\rotationvalue)};
    \def\RTwoOne{+sin(\rotationvalue)};
    \def\RTwoTwo{+cos(\rotationvalue)};
    % obstacle:
    \def\obstDirection{30}
    \def\obstInOtherFrameX{\scalingmajor*cos(\obstDirection)};
    \def\obstInOtherFrameY{\scalingminor*sin(\obstDirection)};
    \def\obstX{\expectedx+\ROneOne*\obstInOtherFrameX+\ROneTwo*\obstInOtherFrameY};
    \def\obstY{\expectedy+\RTwoOne*\obstInOtherFrameX+\RTwoTwo*\obstInOtherFrameY};
    \draw[black] ({\obstX},{\obstY}) circle (\radiusObstacle) node[below right] {obstacle};
    \filldraw    ({\obstX},{\obstY}) circle (1pt);
    % robot:
    \def\botDirection{43}
    \def\botInOtherFrameX{(\scalingmajor+\distance)*cos(\botDirection)};
    \def\botInOtherFrameY{(\scalingminor+\distance)*sin(\botDirection)};
    \def\botX{\expectedx+\ROneOne*\botInOtherFrameX+\ROneTwo*\botInOtherFrameY};
    \def\botY{\expectedy+\RTwoOne*\botInOtherFrameX+\RTwoTwo*\botInOtherFrameY};
    \draw[black] ({\botX},{\botY}) circle (\radiusRobot) node[above right] {robot};
    \filldraw    ({\botX},{\botY}) circle (1pt);
    % intersection:
    \begin{scope}
        \clip({\obstX},{\obstY}) circle (\radiusObstacle);
        \fill[tublau] ({\botX},{\botY}) circle (\radiusRobot);
    \end{scope}
    % draw arrow with error:
    \draw[pfeil, tublau] ({\botX-1.1},{\botY+0.4}) -- ({\botX-0.2},{\botY-0.65}) node[at start, anchor=south east]{\textcolor{tublau}{unwanted intersection}};
\end{tikzpicture}

==> Figures/visual_representation.tex <==
\begin{tikzpicture}
    % variables
    \def\rotationvalue{45}
    \def\expectedx{2}
    \def\expectedy{2}
    \def\scalingminor{1.5}
    \def\scalingmajor{2.5}
    \def\distance{1.3}
    % Draw the coordinate system
    \draw[pfeil] (-1,0) -- (3,0) node[below] {$\prescript{}{0}{x}$};
    \draw[pfeil] (0,-1) -- (0,3) node[left] {$\prescript{}{0}{y}$};
    % Draw the ellipse centered at (1,1)
    \draw[black] (\expectedx,\expectedy) ellipse [x radius=\scalingmajor cm, y radius=\scalingminor cm, rotate=\rotationvalue];
    \fill[chemorange, opacity=0.1] (\expectedx,\expectedy) ellipse [x radius=\scalingmajor cm, y radius=\scalingminor cm, rotate=\rotationvalue];
    \draw[black] (\expectedx,\expectedy) ellipse [x radius={\scalingmajor+\distance}, y radius={\scalingminor+\distance}, rotate=\rotationvalue];
    \fill[wiwirot, opacity=0.1] (\expectedx,\expectedy) ellipse [x radius={\scalingmajor+\distance}, y radius={\scalingminor+\distance}, rotate=\rotationvalue];
    % Optional: grid for reference
    % Draw eigen-vectors
    % major
    \draw[pfeil, wiwirot] (\expectedx,\expectedy) -- ({\expectedx + cos(\rotationvalue)*(\scalingmajor+\distance)}, {\expectedy + sin(\rotationvalue)*(\scalingmajor+\distance)}) node[above, rotate=\rotationvalue] {$\left(s \sqrt{\lambda_a} + r + r_d\right) \prescript{}{0}{\matvar{a}}_{d, k+i}$};
    \draw[pfeil, chemorange] (\expectedx,\expectedy) -- ({\expectedx + cos(\rotationvalue)*\scalingmajor}, {\expectedy + sin(\rotationvalue)*\scalingmajor}) node[below, rotate=\rotationvalue] {$s \sqrt{\lambda_a} \prescript{}{0}{\matvar{a}}_{d, k+i}$};
    \draw[pfeil, black] (\expectedx,\expectedy) -- ({\expectedx + cos(\rotationvalue)}, {\expectedy + sin(\rotationvalue)}) node[above, rotate=\rotationvalue] {$\prescript{}{0}{\matvar{a}}_{d, k+i}$};
    % minor
    \draw[pfeil, wiwirot] (\expectedx,\expectedy) -- ({\expectedx - cos(\rotationvalue)*(\distance+\scalingminor)}, {\expectedx + sin(\rotationvalue)*(\distance+\scalingminor)}) node[above left, rotate=\rotationvalue] {$\left(s \sqrt{\lambda_b} + r + r_d\right) \prescript{}{0}{\matvar{b}}_{d, k+i}$};
    \draw[pfeil, chemorange] (\expectedx,\expectedy) -- ({\expectedx - cos(\rotationvalue)*\scalingminor}, {\expectedx + sin(\rotationvalue)*\scalingminor}) node[above right, rotate=\rotationvalue] {$s \sqrt{\lambda_b} \prescript{}{0}{\matvar{b}}_{d, k+i}$};
    \draw[pfeil, black] (\expectedx,\expectedy) -- ({\expectedx - cos(\rotationvalue)}, {\expectedx + sin(\rotationvalue)}) node[left, rotate=\rotationvalue] {$\prescript{}{0}{\matvar{b}}_{d, k+i}$};
    % draw rotated coordiantes
    \draw[pfeil, black] (\expectedx,\expectedy) -- (\expectedx+1, \expectedy) node[right] {};
    \draw[pfeil, black] (\expectedx,\expectedy) -- (\expectedx, \expectedy+1) node[below left] {};
    % Mark the center of the ellipse
    \fill[wiwirot] (\expectedx,\expectedy) circle (2pt) node[below] {$\matvar{\mu}_{d, k+i}$};
    %
    \node[wiwirot] at (\expectedx-1,\expectedy-2.7) {$\mathbb{D}_{d,k+i}$};
    \node at (4,-1) {$\mathbb{D}_{d,k+i}^\complement$};
\end{tikzpicture}
